Determination of the lightest strange resonance $K_0^*(700)$ or $\kappa$, from a dispersive data analysis

In this work we present a precise and model-independent dispersive determination from data of the existence and parameters of the lightest strange resonance $\kappa/K_0^*(700)$. We use both subtracted and unsubtracted partial-wave hyperbolic and fixed-$t$ dispersion relations as constraints on combined fits to $\pi K\rightarrow\pi K$ and $\pi\pi\rightarrow K\bar K$ data. We then use the hyperbolic equations for the analytic continuation of the isospin $I=1/2$ scalar partial wave to the complex plane, in order to determine the $\kappa/K_0^*(700)$ and $K^*(892)$ associated pole parameters and residues.

==> figures/f12.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1276,3784){\makebox(0,0){\strut{}Re $f^{1/2}_0(s)$}}%
      \put(3764,154){\makebox(0,0){\strut{}$\sqrt{s}$ GeV}}%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}UFD Output}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}UFD Input}}%
      \csname LTb\endcsname%
      \put(594,594){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(594,1117){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \put(594,1639){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(594,2162){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(594,2685){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(594,3207){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(594,3730){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(594,4252){\makebox(0,0)[r]{\strut{}$0.9$}}%
      \put(594,4775){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(967,374){\makebox(0,0){\strut{}$0.65$}}%
      \put(1908,374){\makebox(0,0){\strut{}$0.7$}}%
      \put(2850,374){\makebox(0,0){\strut{}$0.75$}}%
      \put(3791,374){\makebox(0,0){\strut{}$0.8$}}%
      \put(4732,374){\makebox(0,0){\strut{}$0.85$}}%
      \put(5673,374){\makebox(0,0){\strut{}$0.9$}}%
      \put(6615,374){\makebox(0,0){\strut{}$0.95$}}%
      \put(2850,1117){\makebox(0,0){\strut{}$\hat{d}^2=5.7$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{f12}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/f12sub.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1276,3784){\makebox(0,0){\strut{}Re $f^{1/2}_0(s)$}}%
      \put(3764,154){\makebox(0,0){\strut{}$\sqrt{s}$ GeV}}%
      \csname LTb\endcsname%
      \put(5816,987){\makebox(0,0)[r]{\strut{}UFD Output}}%
      \csname LTb\endcsname%
      \put(5816,767){\makebox(0,0)[r]{\strut{}UFD Input}}%
      \csname LTb\endcsname%
      \put(594,594){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(594,1117){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \put(594,1639){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(594,2162){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(594,2685){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(594,3207){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(594,3730){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(594,4252){\makebox(0,0)[r]{\strut{}$0.9$}}%
      \put(594,4775){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(967,374){\makebox(0,0){\strut{}$0.65$}}%
      \put(1908,374){\makebox(0,0){\strut{}$0.7$}}%
      \put(2850,374){\makebox(0,0){\strut{}$0.75$}}%
      \put(3791,374){\makebox(0,0){\strut{}$0.8$}}%
      \put(4732,374){\makebox(0,0){\strut{}$0.85$}}%
      \put(5673,374){\makebox(0,0){\strut{}$0.9$}}%
      \put(6615,374){\makebox(0,0){\strut{}$0.95$}}%
      \put(2850,1117){\makebox(0,0){\strut{}$\hat{d}^2=3.1$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{f12sub}}%
    \gplfronttext
  \end{picture}%
\endgroup

